Differential Privacy Meets Federated Learning under Communication Constraints

The performance of federated learning systems is bottlenecked by communication costs and training variance. The communication overhead problem is usually addressed by three communication-reduction techniques, namely, model compression, partial device participation, and periodic aggregation, at the cost of increased training variance. Different from traditional distributed learning systems, federated learning suffers from data heterogeneity (since the devices sample their data from possibly different distributions), which induces additional variance among devices during training. Various variance-reduced training algorithms have been introduced to combat the effects of data heterogeneity, while they usually cost additional communication resources to deliver necessary control information. Additionally, data privacy remains a critical issue in FL, and thus there have been attempts at bringing Differential Privacy to this framework as a mediator between utility and privacy requirements. This paper investigates the trade-offs between communication costs and training variance under a resource-constrained federated system theoretically and experimentally, and how communication reduction techniques interplay in a differentially private setting. The results provide important insights into designing practical privacy-aware federated learning systems.

==> alg_fedpaq.tex <==
\begin{algorithm}
\caption{FedPaq.}
\label{alg: federated learning}
\begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Initialize:}}
 \newcommand{\algorithmicinitialize}{\textbf{Initialize:}}
 \REQUIRE learning rate $\eta_k$ for $k\in[K]$
 \ENSURE model parameters $\mathbf{x}_0 \in \mathbb{R}^d$
  \FOR {each round $k = [K]$}
  \STATE \textbf{on each device} $i\in\mathcal{S}_k$:
  \begin{ALC@g}
  \STATE Initialize the local model $\mathbf{x}_{k,0}^{(i)} = \mathbf{x}_k$
  \FOR {each iteration $t = 0,\cdots,E-1$}
  \STATE calculate $\mathbf{x}_{k, t+1}^{(i)} = \mathbf{x}_{k, t}^{(i)} - \eta_k \tilde{\nabla} f_i\left(\mathbf{x}_{k,t}^{(i)} \right)$
  \ENDFOR
  \STATE send $\Delta\mathbf{x}_{k}^{(i)} = Q\left(\mathbf{x}_{k,E}^{(i)} - \mathbf{x}_k\right)$ to the server
  \end{ALC@g}
  \STATE \textbf{on the parameter server}:
  \begin{ALC@g}
  \STATE calculate $\mathbf{x}_{k+1} = \mathbf{x}_k +  \frac{1}{M}\sum_{i\in\mathcal{S}_k}\Delta\mathbf{x}_{k}^{(i)}$ 
  \STATE broadcast the global model $\mathbf{x}_{k+1}$ to all devices
  \end{ALC@g}
  \ENDFOR
  
\end{algorithmic} 
\end{algorithm}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
